Predicting the Target Word of Game-playing Conversations using a Low-Rank Dialect Adapter for Decoder Models

Dialect adapters that improve the performance of LLMs for NLU tasks on certain sociolects/dialects/national varieties ('dialects' for the sake of brevity) have been reported for encoder models. In this paper, we extend the idea of dialect adapters to decoder models in our architecture called LoRDD. Using MD-3, a publicly available dataset of word game-playing conversations between dialectal speakers, our task is Target Word Prediction (TWP) from a masked conversation. LoRDD combines task adapters and dialect adapters where the latter employ contrastive learning on pseudo-parallel conversations from MD-3. Our experiments on Indian English and Nigerian English conversations with two models (Mistral and Gemma) demonstrate that LoRDD outperforms four baselines on TWP. Additionally, it significantly reduces the performance gap with American English, narrowing it to 12% and 5.8% for word similarity, and 25% and 4.5% for accuracy, respectively. The focused contribution of LoRDD is in its promise for dialect adaptation of decoder models using TWP, a simplified version of the commonly used next-word prediction task.

==> sections/commentedtext.tex <==
\begin{table*}[ht!]
    \centering
    \begin{adjustbox}{width=1.0\linewidth,center}
        \renewcommand{\arraystretch}{1.1}
        \setlength{\cmidrulekern}{0.25em}
        \begin{tabular}{%
        m{12em}
        m{6em}
        m{4em}
        *{4}{S[table-format=1]}
        }
        \toprule
        \multirow{2}{12em}{Method} & \multirow{2}{6em}{Train Data} & \multirow{2}{4em}{Test Data} & \multicolumn{2}{c}{\mistral} & \multicolumn{2}{c}{\gemma} \\\cmidrule(lr){4-5}\cmidrule(lr){6-7}
        & & & Similarity & Accuracy & Similarity & Accuracy\\\midrule[\heavyrulewidth]
        In-dialect \small{(Skyline)} & \USEng & \USEng & 64.7 & 44.3 & 69.7 & 45.3 \\
        In-dialect \small{(Baseline \#1)} & \IndEng &\IndEng & 51.0 & 24.4 & 54.6 & 30.0 \\\hdashline
        %Cross-dialect \small{(Baseline \#2)} & \USEng & \IndEng & 54.6 & 25.6 & 61.3 & 35.0 \\\hdashline
        Our Method & Custom & \IndEng & 55.9 & 30.0 & 62.8 & 38.8\\
        \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:baselines}}
\end{table*}
\begin{table*}[ht!]
    \centering
    \begin{adjustbox}{width=1.0\linewidth,center}
        \renewcommand{\arraystretch}{1.1}
        \setlength{\cmidrulekern}{0.25em}
        \begin{tabular}{m{4em}m{4em}m{3em}cccccc}
        \toprule
        
        &\multirow{2}{4em}{Method} & \multirow{2}{3em}{Dataset} & \multicolumn{2}{c}{\mistral} & \multicolumn{2}{c}{\gemma} & \multicolumn{2}{c}{$\mathbf{\Delta}$}\\\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
         && & Similarity($\uparrow$) & Accuracy($\uparrow)$ & Similarity($\uparrow$) & Accuracy($\uparrow)$ & Similarity($\downarrow$) & Accuracy($\downarrow)$\\\midrule[\heavyrulewidth]
         \multirow{2}{4em}{\texttt{COMP9991}} & FT & \USEng & 64.7 & 44.3 & 69.7 & 45.3 & - & - \\
          & FT & \IndEng & 51.0 & 24.4 & 54.6 & 30.0 & 14.4 & 17.6\\\hdashline
          \texttt{COMP9993} & \multicolumn{2}{c}{\texttt{Ours}}& 55.9 \small{(+4.9)} & 30.0 \small{(+5.6)} & 62.8 \small{(+8.3)} & 38.8 \small{(+8.8)} & 7.9 \small{(-6.5)} &  10.4 \small{(-7.2)}\\
        \bottomrule
        %& 13.7 & 19.9
        \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:baselines}
    \textbf{Performance Improvement on Target Word Prediction.} For each model, we report Similarity and Accuracy ($\uparrow$, higher the better) for both approaches -- fine-tuning (FT) and proposed (Ours). $\Delta$ is the average performance degradation across both models on \IndEng compared to \USEng (\USEng minus \IndEng $\downarrow$, lower the better). Performance improvement is shown by the number in parenthesis.
    }
\end{table*}

\begin{table*}[ht!]
    \centering
    \begin{adjustbox}{width=1.0\linewidth,center}
        % \renewcommand{\arraystretch}{1.1}
        \setlength{\cmidrulekern}{0.25em}
        \begin{tabular}{m{6em}m{6em}cccccc}
        \toprule
        \multirow{3}{6em}{Method} & \multirow{3}{6em}{Test Dialect} & \multicolumn{2}{c}{\mistral} & \multicolumn{2}{c}{\gemma}&\multicolumn{2}{c}{$\mu$}\\\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
         & & Similarity & Accuracy & Similarity & Accuracy & Similarity & Accuracy\\\midrule[\heavyrulewidth]
         FT w/ \USEng & \USEng & 64.7 & 44.3 & 69.7 & 45.3 & 67.2 & 44.8\\\hdashline
         FT w/ \USEng & \multirow{3}{6em}{\IndEng} & 54.6\improve{} & 25.6\improve{} & 61.3\improve{} & 35.0\improve{} & 58.0\improve{} & 30.3\improve{}\\
         FT w/ \IndEng &  & 51.0 & 24.4 & 54.6 & 30.0 & 52.8 & 27.2\\
         FT w/ \Multi &  & 52.4\improve{} & 24.4 & 58.2\improve{} & 30.0 & 55.3\improve{} & 27.2\\\hdashline
         \ours & \IndEng & 55.9\improve{} & 30.0\improve{} & 63.9\improve{} & 41.3\improve{} & 59.4\improve{} & 34.4\improve{}\\
         % $\Delta$ ($\downarrow$) & 13.7 & 8.9 \small{(-4.9)}& 19.9 & 14.3 \small{(-5.6)}& 15.1 & 6.9 \small{(-8.3)}& 15.3 & 6.5 \small{(-8.8)}& 14.4 & 7.9 \small{(-6.6)}& 17.6 & 10.4 \small{(-7.2)}\\
         % \multicolumn{2}{c}{\texttt{Ours}}& 55.9 & 30.0 & 62.8 & 38.8 & 7.9 &  10.4\\\hdashline
         
        \bottomrule
        %& 13.7 & 19.9
        \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:baselines}
    \textbf{Baselines.} For each model, we report Similarity and Accuracy for both approaches -- only fine-tuning (FT) and proposed (\ours). $\mu$ is the average of the metrics across both models. Performance improvement compared to \IndEng is shown by \improve{}.
    }
\end{table*}

\begin{table*}[ht!]
    \centering
    \begin{adjustbox}{width=1.0\linewidth,center}
        % \renewcommand{\arraystretch}{1.1}
        \setlength{\cmidrulekern}{0.25em}
        \begin{tabular}{m{10em}cccccc}
        \toprule
        \multirow{2}{10em}{Method} & \multicolumn{2}{c}{\mistral} & \multicolumn{2}{c}{\gemma} & \multicolumn{2}{c}{$\mu$}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
          & Similarity & Accuracy & Similarity & Accuracy & Similarity & Accuracy\\\midrule[\heavyrulewidth]
         % \ours & 55.9 & 30.0 & 62.8 & 38.8 & 59.4 & 34.4\\\hdashline
         FT w/ \IndEng & 51.0 & 24.4 & 54.6 & 30.0 & 52.8 & 27.2\\\hdashline
         % FT w/ \USEng & 54.6 & 25.6 & 61.3 & 35.0\\
         % FT w/ \Multi & 52.4 & 24.4 & 58.2 & 30.0\\\hdashline
         FT w/ \USEng + \IndEng & \textbf{54.4} & \textbf{26.9} & \textbf{62.3} & \textbf{37.5} & \textbf{58.4} & \textbf{32.2}\\
         FT w/ \Trans + \IndEng & 44.8 & 18.1 & 57.5 & 28.8 & 51.2 & 23.5\\
         FT w/ \Multi + \IndEng & 51.6 & 23.1 & 57.1 & 31.9 & 54.4 & 27.5\\
        \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:baselines}
    \textbf{Data Augmentation.} For each model, we report Similarity and Accuracy when tested on \IndEng. $\mu$ is the average performance across both models. The best performance for all configurations is represented by \textbf{bold} numbers.
    }
\end{table*}


\begin{table*}[h!]
    \centering
    \begin{adjustbox}{width=1.0\linewidth,center}
        % \renewcommand{\arraystretch}{1.1}
        % \setlength{\cmidrulekern}{0.25em}
        \begin{tabular}{llc}
        \toprule
         \textbf{Feature} & \textbf{Example} & \textbf{Count}\\\midrule[\heavyrulewidth]
         \textsc{extraneous article} & \emph{you can combine \underline{the} both the words} & 11\\
         \textsc{lack of inversion in wh-questions} & \emph{What \underline{you are} using right now?} & 6\\
         \textsc{left dislocation} & \emph{\underline{If we have a five sides}, what do we call that?} & 6\\
         \textsc{article omission} & \emph{I'll explain you (the) second word} & 5\\
         \textsc{object fronting} & \emph{\underline{some towers type} it will be} & 5\\
         \textsc{focus} \emph{only} & \emph{I'm trying to explain that \underline{only}} & 3\\
         \textsc{non-initial existential} & \emph{brand names also \underline{there}} & 2\\
         \textsc{mass nouns as count nouns} & \emph{How the women\underline{s} will be?} & 2\\
         \textsc{invariant tag} & \emph{put them on some type of wire \underline{no?}} & 1\\
        \bottomrule
        %& 13.7 & 19.9
        \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:dial_feat} Dialect features identified in erroneously labelled \IndEng conversations with the corresponding examples.}
\end{table*}


% We train \ours in two phases. In the first phase, task adapters are trained by fine-tuning \mistral and \gemma for \texttt{20} epochs, with a batch size of \texttt{32}, Paged 8-bit AdamW~\cite{dettmers20228bit} as the optimiser and learning rate of \texttt{2e-4}. We use LoRA adapters, targeting all linear layers, as recommended by~\citet{dettmers2023qlora}. In the second phase, we train dialect adapters using contrastive learning. We employ LoRA adapters similar to task adapters, for \texttt{10} epochs, with a batch size of \texttt{8}, AdamW as the optimiser, learning rate of \texttt{2e-5} and margin of \texttt{0.3}.

